EvoVGM: a Deep Variational Generative Model for Evolutionary Parameter Estimation

Most evolutionary-oriented deep generative models do not explicitly consider the underlying evolutionary dynamics of biological sequences as it is performed within the Bayesian phylogenetic inference framework. In this study, we propose a method for a deep variational Bayesian generative model (EvoVGM) that jointly approximates the true posterior of local evolutionary parameters and generates sequence alignments. Moreover, it is instantiated and tuned for continuous-time Markov chain substitution models such as JC69, K80 and GTR. We train the model via a low-variance stochastic estimator and a gradient ascent algorithm. Here, we analyze the consistency and effectiveness of EvoVGM on synthetic sequence alignments simulated with several evolutionary scenarios and different sizes. Finally, we highlight the robustness of a fine-tuned EvoVGM model using a sequence alignment of gene S of coronaviruses.

==> tab_tex/gtr_b.tex <==
% \vskip -0.1in
\begin{table}[]
\caption{Distance and correlation between actual and estimated branch lengths by EvoVGM\_GTR. Rows correspond to the number of sequences. Columns correspond to the alignment length.}
\label{tab:gtr_b}
% \vskip -0.1in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{llllllllll}
\toprule
{} & \multicolumn{3}{l}{100} & \multicolumn{3}{l}{1000} & \multicolumn{3}{l}{5000} \\
{} &  dist &  corr &  pval &  dist &  corr &  pval &  dist &  corr &  pval \\
\midrule
3 & 0.300 & 0.984 & 0.114 & 0.090 & 0.980 & 0.126 & 0.097 & 0.986 & 0.107 \\
4 & 0.076 & 0.994 & 0.006 & 0.086 & 0.998 & 0.002 & 0.085 & 0.992 & 0.008 \\
5 & 0.081 & 0.986 & 0.002 & 0.069 & 0.995 & 0.000 & 0.116 & 0.962 & 0.009 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in %%
\end{table}
% Datasets were simulated with GTR substitution model.

==> tab_tex/gtr_f.tex <==
% GTR freqs
\begin{table}[]
\caption{Distance and correlation between actual and estimated relative frequencies by EvoVGM\_GTR.}
\label{tab:gtr_f}
% \vskip 0.1in %%%
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{llllllllll}
\toprule
{} & \multicolumn{3}{l}{100} & \multicolumn{3}{l}{1000} & \multicolumn{3}{l}{5000} \\
{} &  dist &  corr &  pval &  dist &  corr &  pval &  dist &  corr &  pval \\
\midrule
3 & 0.190 & 0.941 & 0.059 & 0.084 & 0.991 & 0.009 & 0.095 & 0.992 & 0.008 \\
4 & 0.125 & 0.891 & 0.109 & 0.090 & 0.996 & 0.004 & 0.050 & 0.999 & 0.001 \\
5 & 0.176 & 0.775 & 0.225 & 0.022 & 1.000 & 0.000 & 0.033 & 0.999 & 0.001 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in  %%%
\end{table}
% Datasets were simulated with GTR model.

==> tab_tex/gtr_r.tex <==
% GTR rates
\begin{table}[]
\caption{Distance and correlation between actual and estimated substitution rates by EvoVGM\_GTR.}
\label{tab:gtr_r}
% \vskip -0.1in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{llllllllll}
\toprule
{} & \multicolumn{3}{l}{100} & \multicolumn{3}{l}{1000} & \multicolumn{3}{l}{5000} \\
{} &  dist &  corr &  pval &  dist &  corr &  pval &  dist &  corr &  pval \\
\midrule
3 & 0.621 & 0.103 & 0.846 & 0.177 & 0.668 & 0.147 & 0.129 & 0.784 & 0.065 \\
4 & 0.305 & 0.472 & 0.344 & 0.114 & 0.864 & 0.027 & 0.036 & 0.985 & 0.000 \\
5 & 0.206 & 0.652 & 0.160 & 0.053 & 0.968 & 0.002 & 0.012 & 0.998 & 0.000 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in  %%%
\end{table}
%  Datasets were simulated with GTR model.
